Practitioner Trajectories of Engagement with Ethics-Focused Method Creation

Design and technology practitioners are increasingly aware of the ethical impact of their work practices, desiring tools to support their ethical awareness across a range of contexts. In this paper, we report on findings from a series of co-design workshops with technology and design practitioners that supported their creation of a bespoke ethics-focused action plan. Using a qualitative content analysis and thematic analysis approach, we identified a range of roles and process moves that practitioners employed and illustrate the interplay of these elements of practitioners' instrumental judgment through a series of three cases, which includes evolution of the action plan itself, the ethical dilemmas or areas of support the action plan was intended to support, and how the action plan represents resonance for the practitioner that created it. We conclude with implications for supporting ethics in socio-technical practice and opportunities for the further development of ethics-focused methods that are resonant with the realities of practice.

==> participanttable.tex <==
\begin{table*}[!htb]
 \centering
    \begin{tabularx}{\textwidth}{p{.15\textwidth}Xrr}
    \toprule
    \textbf{Name} & \textbf{Professional Title} & \textbf{Years of Experience} & \textbf{Current Company} \\
    \midrule
    PS01A & Product Manager & 3 & Enterprise (B2B2C)\\
    PS01B & UX Designer/Architect/Engineer & 2 & Enterprise (B2B2C)\\
    PS01C & UX Designer/Architect/Engineer & 2 & Enterprise (B2B)\\
    PS01D & UX Researcher & 1 & - \\
    PS02A & UX Designer & 2 & Enterprise (B2B2C)\\
    PS02B & UX Designer/ & 3 & Enterprise (B2B2C)\\
    PS02C & UX Research Lead & 5 & Enterprise (B2B)\\
    PS03A & UX Designer/Architect/Engineer & 2 & Agency or Consultancy\\
    PS03B & Data Scientist & 8 & Enterprise (B2B2C)\\
    PS03C & Data Engineer & 3 & Enterprise (B2C)\\
    PS03D & Product Manager & 10 & Agency or Consultancy\\
    PS03E & UX Designer/Architect/Engineer & 2 & Agency or Consultancy\\
    PS03F & Software Engineer & 5 & Enterprise (B2B2C)\\
    SS01A & UX Designer & - & -\\
    SS01B & UX Designer & - & - \\
    SS01C & UX Designer & - & -\\
    SS01D & UX Researcher & - & -\\
    SS02A & UX Designer/Architect/Engineer & - & -\\
    SS02B & UX Designer/Architect/Engineer & - & -\\
    SS02C & Product Manager & - & -\\
    SS02D & UX Designer/Architect/Engineer & - & -\\
    SS03A & Product Manager & - & -\\
    SS03B & UX Designer/Architect/Engineer & - & -\\
    SS03C & UX Designer/Architect/Engineer & - & -\\
    SS03C & UX Designer & - & -\\
    SS03E & UX Designer/Architect/Engineer & - & -\\    
    \bottomrule
    \end{tabularx}
     \caption{Participants for each section of the co-creation sessions}
     \label{participants}
\end{table*}
